Neural networks are more modular than single neurons suggest

Neural networks routinely develop representations in which individual neurons contribute to multiple distinct functions, leading to the widespread view that such networks lack modular organization. We challenge this conclusion by introducing a formally nested hierarchy of modularity: unit-level, which requires distinct computations to occupy disjoint neurons; orthogonal, which asks whether a rotation reveals functionally independent subspaces; and linear, which asks whether a bounded linear map can separate task-relevant computations into independent subspaces. We develop a unified framework for learning decompositions at each level and evaluating them causally through selective ablation. Across vision models, language models and multi-task Recurrent Neural Networks (RNNs), we find that networks which lack unit-level modularity nonetheless often exhibit clear functional modularity at the subspace level. In vision and language models, content versus style and syntax versus semantics respectively dissociate under subspace ablation despite sharing overlapping populations of neurons. These learned subspaces also align differentially with brain data, with content and style subspaces predicting higher and lower visual cortex respectively, and semantic subspaces outperforming syntactic ones in predicting language cortex activity. In RNNs trained on multiple cognitive tasks and previously shown to lack modular structure, our decomposition recovers sharp double dissociations between tasks. The absence of unit-level modularity frequently coexists with clear subspace-level modularity across domains, enabling targeted intervention on specific computations even in networks where no individual neuron is specialized, with broad implications for mechanistic interpretability and for understanding functional organization in both biological and artificial neural systems.

==> rnn.tex <==
% \subsection{Modularity in recurrent neural networks trained on cognitive tasks}
% \label{sec:rnn_results}
% We apply our modularity hierarchy to two well-studied RNN paradigms from computational neuroscience: the context-dependent integration task of \citet{mante2013context} and the multitask cognitive paradigm of \citet{yang2019task}. Both involve continuous-time recurrent networks (CTRNNs) with 256 units, and both have been central to debates about whether neural networks organize their computations modularly or distribute them across the full population. 

% \paragraph{Measuring functional modularity}
% We evaluate decompositions through causal ablation: zeroing out each subspace during inference and measuring the accuracy drop on both tasks. A double dissociation requires that ablating subspace $A$ selectively impairs one task while ablating subspace $B$ selectively impairs the other. We quantify this with the double dissociation index:
% \begin{equation}
%     \text{DDI} = \max\!\Big(\min(\Delta^\text{sel}_1,\, \Delta^\text{sel}_2) - \max(\Delta^\text{col}_1,\, \Delta^\text{col}_2),\; 0\Big),
%     \label{eq:ddi}
% \end{equation}
% where $\Delta^\text{sel}_i$ is the on-target accuracy drop for task $i$ and $\Delta^\text{col}_i$ is the off-target (collateral) drop. DDI is positive only when both ablations selectively impair their respective tasks more than they damage the other, and approaches 1 for perfect dissociations.



\paragraph{Context-dependent integration (Mante task).}
We trained CTRNNs on the task of \citet{mante2013context}, in which the network receives noisy motion and color evidence simultaneously and must report either the motion or color direction depending on a binary context signal (Figure~\ref{fig:mante}a,b). Networks were trained with tanh activations across 10 random seeds. At the unit level, individual neurons respond to mixtures of motion, color, and context \citep{mante2013context, rigotti2013importance}. We applied our decomposition hierarchy and evaluated the resulting subspaces through causal ablation: zeroing out the motion subspace during inference and measuring the impact on motion versus color decisions, and vice versa.
 
Unit-level and orthogonal decompositions produce near-zero DDI across all subspace dimensions tested ($d_A = d_B \in \{2, 5, 10, 15, 20, 50\}$), confirming that no permutation or rotation of the representation reveals functionally separable components (Figure~\ref{fig:mante}c). In contrast, linear decomposition yields robust double dissociations. At $d = 15$, the linear decomposition achieves DDI $= 0.277 \pm 0.026$ (mean $\pm$ s.d. across seeds): ablating the motion subspace reduces motion accuracy by ${\sim}39\%$ while leaving color accuracy nearly intact (collateral $< 4\%$), and ablating the color subspace produces the symmetric pattern (Figure~\ref{fig:mante}a,b). The DDI increases with subspace dimension up to $d \approx 15$--$20$ and plateaus thereafter (Figure~\ref{fig:mante}c), indicating that the functionally relevant subspaces are low-dimensional relative to the full 256-dimensional representation.

As a baseline, we also applied targeted dimensionality reduction (TDR) \citep{mante2013context}, which identifies the single axis in representation space along which activity best predicts each task variable via linear regression. TDR successfully identifies motion and color axes with high predictive accuracy ($R^2 = 0.77 \pm 0.01$ and $0.76 \pm 0.01$ respectively) that are approximately orthogonal (cosine similarity $= -0.03 \pm 0.10$), consistent with the original findings of \citet{mante2013context}. However, ablating these axes during inference has negligible causal effect: accuracy drops by less than $0.5\%$ for both tasks across all 10 seeds. This dissociation between predictive and causal relevance indicates that while motion and color information is correlated with these single axes, the functionally necessary computation is distributed across a higher-dimensional subspace. Our linear decomposition, which identifies multi-dimensional subspaces optimized for task sufficiency, recovers the causal structure that single-axis methods miss. The contrast also highlights a key distinction: encoding information along a direction is not the same as depending on that direction for computation.


% \begin{figure}[t]
% \centering
% \includegraphics[width=0.8\textwidth]{fig_mante_main_final.png}
% \caption{\textbf{Functional modularity in the Mante et al. (2013) context-dependent integration RNN.}
% \textbf{(a,b)}~Accuracy on motion and color tasks after ablating the motion or color subspace (linear decomposition, $d=50$), shown for unit, orthogonal, and linear levels. Horizontal lines indicate intact baseline accuracy. Only linear decomposition produces selective impairment.
% \textbf{(c)}~DDI as a function of subspace dimension for unit (gray), orthogonal (blue), and linear (red) decompositions. Unit and orthogonal DDI remain near zero at all dimensions; linear DDI rises to $\sim$0.28 by $d=15$.
% \textbf{(d)}~Accuracy after ablation as a function of dimension (linear decomposition). Solid lines show the targeted task (which should drop); dashed lines show the spared task (which should remain high). The dissociation emerges progressively with increasing subspace dimension.}
% \label{fig:mante}
% \end{figure}

% \paragraph{Multitask cognitive RNNs (Yang task).}

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.9\textwidth]{fig_yang_modularity_final.png}
% \caption{\textbf{Functional modularity in multitask RNNs (Yang et al., 2019).}
% \textbf{(a,f)}~FTV distributions for Anti vs DM1 in softplus (top) and tanh (bottom) networks. Softplus shows bimodal clustering; tanh shows a broad unimodal distribution centered near zero.
% \textbf{(b--e)}~Double dissociation bars for softplus networks at each hierarchy level (unit, Sinkhorn, orthogonal, linear). All levels show selective ablation effects (DDI = 0.59--0.73).
% \textbf{(g--j)}~Same for tanh networks. Unit-level DDI=0.00; orthogonal DDI = 0.37; linear DDI = 0.47. Subspace decomposition recovers modularity that is invisible at the unit level.
% \textbf{(k)}~Negative controls: inclusive (DM1 vs DlyDM1) and mixed (DM1 vs CtxDM1) pairs in both activations, using orthogonal decomposition at $d=25$. Both ablations cause large accuracy drops, but non-selectively (DDI = 0.00 because collateral damage is always greater than selective impairment), confirming that the method does not fabricate modularity where computation is genuinely shared.}
% \label{fig:yang}
% \end{figure}
% We next applied our hierarchy to networks trained on 11 cognitive tasks spanning sensorimotor mapping, perceptual decision-making, context-dependent integration, working memory, and categorical matching \citep{yang2019task}. We trained networks with both softplus and tanh activations. Following the taxonomy of \citet{yang2019task}, we evaluate three task pairs that span the spectrum from fully separable to fully shared computation:
 
% \begin{itemize}[nosep,leftmargin=*]
% \item \textbf{Anti vs DM1 (disjoint):} Anti requires responding in the opposite direction of a single stimulus (sensorimotor remapping), while DM1 requires reporting which of two overlapping stimuli is stronger (perceptual evidence comparison). These tasks share no computational requirements.
% \item \textbf{DM1 vs DlyDM1 (inclusive):} DlyDM1 performs the same comparison as DM1 but with a delay between stimuli, requiring additional working memory. DlyDM1 is computationally a superset of DM1.
% \item \textbf{DM1 vs CtxDM1 (mixed):} CtxDM1 presents stimuli on both input modalities but must selectively attend to one based on a context cue, using DM1's comparison machinery plus context-dependent input gating. The two tasks share their core computation.
% \end{itemize}
 
% Figure~\ref{fig:yang} first shows results for the disjoint pair (Anti vs DM1). We begin with the fractional task variance (FTV) analysis introduced by \citet{yang2019task}, which measures, for each unit, the relative variance contributed by each task. In softplus networks, the FTV distribution is strongly bimodal ($|\text{FTV}| = 0.74$, with 74\% of units specialized for one task), indicating that Anti and DM1 are supported by largely non-overlapping populations (Figure~\ref{fig:yang}a). In tanh networks, the FTV distribution is broad and unimodal ($|\text{FTV}| = 0.39$, 30\% specialized), with most units contributing similarly to both tasks (Figure~\ref{fig:yang}f). This is the observation that led \citet{yang2019task} to conclude that tanh networks lack modular structure and that ``state-space approaches may be more appropriate'' for their analysis.
 
% Our decomposition hierarchy reveals interesting trends. In softplus networks, all levels recover a double dissociation, with DDI increasing from unit (0.59) through orthogonal (0.73) to linear (0.70) (Figure~\ref{fig:yang}b--e). The strong FTV clustering means that even the simplest decomposition (assigning units to tasks based on their FTV values) produces selective ablation effects, consistent with the cluster-based lesioning results reported by \citet{yang2019task}. The critical result is in tanh networks. Unit-level decomposition yields DDI $= 0.00$: despite the FTV identifying some weakly specialized units, ablating them produces collateral damage that overwhelms their selective effects (Figure~\ref{fig:yang}g). Sinkhorn permutation, which searches for a better unit assignment than FTV ranking, yields only DDI $= 0.08$. But orthogonal decomposition achieves DDI $= 0.37$ (Figure~\ref{fig:yang}i), and linear decomposition reaches DDI $= 0.47$ (Figure~\ref{fig:yang}j), recovering a clear double dissociation in a network where unit-level analysis finds no modular structure. This confirms the hypothesis of \citet{driscoll2024flexible} that such networks possess functional structure ``not aligned to unit axes.''
 
% For the negative control pairs, such as inclusive (DM1 vs DlyDM1) and mixed (DM1 vs CtxDM1), all levels of the hierarchy yield DDI $= 0$ in both activation conditions (Figure~\ref{fig:yang}k). Both ablations cause accuracy drops, but the drops are non-selective and impair both tasks roughly equally. The method correctly identifies that no subspace decomposition can selectively impair one task without equally affecting the other, confirming that it does not fabricate modularity where computation is genuinely shared.
 
Together, the Mante and Yang results establish two key findings. First, the modularity hierarchy reveals structure that unit-level analyses miss: networks that appear non-modular under conventional analysis harbor clear functional modularity at the subspace level. Second, the level at which modularity emerges depends on the network's computational organization: softplus networks are modular at all levels including unit, while tanh networks require orthogonal or linear decomposition to expose the same functional separation.

